Sparse and spurious: dictionary learning with noise and outliers

A popular approach within the signal processing and machine learning communities consists in modelling signals as sparse linear combinations of atoms selected from a learned dictionary. While this paradigm has led to numerous empirical successes in various fields ranging from image to audio processing, there have only been a few theoretical arguments supporting these evidences. In particular, sparse coding, or sparse dictionary learning, relies on a non-convex procedure whose local minima have not been fully analyzed yet. In this paper, we consider a probabilistic model of sparse signals, and show that, with high probability, sparse coding admits a local minimum around the reference dictionary generating the signals. Our study takes into account the case of over-complete dictionaries, noisy signals, and possible outliers, thus extending previous work limited to noiseless settings and/or under-complete dictionaries. The analysis we conduct is non-asymptotic and makes it possible to understand how the key quantities of the problem, such as the coherence or the level of noise, can scale with respect to the dimension of the signals, the number of atoms, the sparsity and the number of observations.

==> mainresults.tex <==
%!TEX root =  sparse_and_spurious.tex

\section{Detailed Statements of the Main results}
We gather in this appendix the detailed statements and the proofs of the simplified results presented in the core of the paper.
In particular, we show in this section that under appropriate scalings of the problem dimensions $(m,p)$, number of training samples $n$, and model parameters $k,\loweralpha,\sigma_{\alpha},\sigma,\mu_0$, it is possible to prove that, with high probability,
the problem of sparse coding admits a local minimum in a certain neighborhood of $\Dbo$ of controlled size, for appropriate choices of the regularization parameter $\lambda$.
%
%
\subsection{Minimum local of sparse coding}\label{sec:minimum_sparsecoding}
We present here a complete and detailed version of our result upon which the theorems presented in the paper are built.
\begin{theorem}[Local minimum of sparse coding]
\label{th:minimum_sparsecoding}
Let us consider our generative model of signals for some reference dictionary $\Dbo \in \Real^{m \times p}$ with coherence $\mu_0$.
Introduce the parameters 
$
q_\alpha \defin \frac{\Exp[\alpha^2]}{\sigma_\alpha^2}
$
and
$
\Qcal_\alpha \defin \frac{\Exp[\alpha^2]}{\sigma_\alpha\cdot\Exp[|\alpha|]}
$
which depend on the distribution of $\alphabo$ only.
Consider the following quantities:
\begin{eqnarray*}
\tau = \tau(\Dbo,\alphabo) &\defin& \min\Big\{ \frac{\loweralpha}{ \sigma_\alpha}, 
\frac{1}{3c_0}\cdot \frac{\Qcal_\alpha}{k \triple \Dbo \triple_2}\Big\}\\
\gamma = \gamma(n,\Dbo,\alphabo) &\defin& 
\frac{1}{2} \min\Bigg\{\sqrt{2\log(n)},
\frac{1}{2\sqrt{2} c_0 c_\gamma} \cdot 
\frac{\Qcal_\alpha}{\triple \Dbo \triple_2 \cdot k \mu_0}
\Bigg\},
\end{eqnarray*}
and let us define the radius $t \in \Real_+$ by 
$$
t \defin 
\max\bigg\{
\frac{4\sqrt{2} c_\gamma}{q_\alpha} \cdot p \cdot\Big\{ c_1 \gamma^3 e^{-\gamma^2} + 2c_2\cdot \gamma\cdot \Big[ m p \frac{\log(n)}{n}\Big]^{1/2}\Big\},  
\frac{\sigma}{\sigma_\alpha}\cdot \sqrt{m}\bigg\}
$$
for some universal constants $c_{*}$.
Provided the following conditions are satisfied:
\begin{itemize}
 \item[]\textbf{(Coherence)} \hspace*{1.5cm}
$\displaystyle
\triple \Dbo \triple_2 \cdot k \mu_0
\leq 
\frac{1}{4\sqrt{2} c_0 c_\gamma}\cdot \frac{\Qcal_\alpha}
{\sqrt{\log( 69 c_1 c_\gamma^2 \cdot \frac{1}{q_\alpha} 
\cdot \frac{p}{\tau}  )}},
$
 \item[]\textbf{(Sample complexity)}
$\displaystyle\
 \frac{\log(n)}{n} \leq 
\frac{q_\alpha^2}{c_3} \cdot 
\frac{1}{m\cdot p^3} \cdot
\frac{\tau^2}{\gamma^4},
$
\end{itemize}
one can find a regularization parameter 
$
\lambda
$
proportional to
$ 
\gamma \cdot \sigma_{\alpha} \cdot  t
$, 
and with probability exceeding
$$
1 - \Big(\frac{mpn}{9}\Big)^{-\frac{mp}{2}} - e^{-4\sqrt{n}},
$$
there exists a local minimum in 
$
\Big\{ \Db \in \Dcal;\ \|\Dbo-\Db\|_\fro < t  \Big\}.
$ 
\end{theorem}
As it will discussed at greater length in Sec.~\ref{sec:building_blocks}, 
we can see that the probability of success of Theorem~\ref{th:minimum_sparsecoding}
can be decomposed into the contributions of the concentration of the surrogate function and the residual term. 
We next present a second result which assumes a more constrained signal model:
\begin{theorem}[Local minimum of sparse coding with noiseless/bounded signals]\label{th:minimum_sparsecoding_simple}
Let us consider our generative model of signals for some reference dictionary $\Dbo \in \Real^{m \times p}$ with coherence $\mu_0$.
Further assume that $\alphabo$ is almost surely upper bounded by $\upperalpha$ and that there is no noise, that is, $\sigma =0$.
Introduce the parameters 
$
q_\alpha \defin \frac{\Exp[\alpha^2]}{\upperalpha\cdot\Exp[|\alpha|]}
$
and 
$
\Qcal_\alpha \defin \frac{\Exp[\alpha^2]}{\sigma_\alpha\cdot\Exp[|\alpha|]}
$
which depend on the distribution of $\alphabo$ only.
Consider the radius $t \in \Real_+$: 
$$
t \defin \frac{8 c_1 c_\lambda}{q_\alpha}
\bigg[ k m p^3\cdot \frac{\log(n)}{n} \bigg]^{1/2}
$$
for some universal constants $c_{*}$.
Provided the following conditions are satisfied:
\begin{itemize}
 \item[]\textbf{(Coherence)} \hspace*{1.5cm}
$\displaystyle\triple \Dbo \triple_2\cdot k^{3/2}\mu_0 
\leq 
\frac{1}{c_0 c_\lambda} \cdot q_\alpha$ 
 \item[]\textbf{(Sample complexity)}
$\displaystyle\
\frac{\log(n)}{n} \leq 
\frac{1}{k^2 m p^3} \cdot \bigg[\frac{\Exp[\alpha^2]}{\upperalpha^2} \cdot \frac{1}{9 c_1 c_\lambda^2}
\cdot  
\min\bigg\{ \frac{\loweralpha}{\sigma_\alpha}, \frac{1}{5c_0} \cdot \frac{\Qcal_\alpha}{k \cdot \triple \Dbo \triple_2} \bigg\} \bigg]^{2},
$
\end{itemize}
one can find a regularization parameter $\lambda$ proportional to $\sqrt{k}\cdot \upperalpha\cdot t$, 
and with probability exceeding
$$
1 - \Big(\frac{mpn}{9}\Big)^{-mp/2},
$$
there exists a local minimum in 
$
\Big\{ \Db \in \Dcal;\ \|\Dbo-\Db\|_\fro < t  \Big\}.
$
\end{theorem}
%
%
These two theorems, which are proved in Section~\ref{app:minimum_sparsecoding}, heavily relies on the following central result.
\subsection{The backbone of the analysis}\label{sec:main_result}
%
%
We concentrate on the result which constitutes the backbone of our analysis. Indeed, we next show how the difference
\begin{equation}
\label{eq:DefDeltaFn}
\Delta F_{n}(\Wb,\vb,t) \defin F_{n}(\Db(\Wb,\vb,t)) - F_{n}(\Dbo).
\end{equation}
is lower bounded with high probability and uniformly with respect to all possible choices of the parameters $(\Wb,\vb)$. 
The theorem and corollaries displayed in the core of the paper are consequences of this general theorem, 
discussing under which conditions/scalings this lower bound can be proved to be sufficient (i.e., strictly positive)
to exploit Proposition~1 and conclude to the existence of a local minimum for $t$ appropriately chosen. 
We define
\begin{equation}
\label{eq:DefCrho}
Q_t  \defin  \frac{1}{\sqrt{1-k\mu(t)}}\quad \text{and}\quad C_t  \defin  \frac{1}{\sqrt{1-\delta_k(\Dbo)}-t},
\end{equation}
where the quantity $\delta_k(\Dbo)$ is the RIP constant itself defined in Section~\ref{app:RIP}.
%
%
\begin{theorem}
\label{th:control_Fn}
Let $\loweralpha,\sigma_{\alpha}$ be the  parameters of the coefficient model.  
Consider $\Dbo$ a dictionary in $\Real^{m \times p}$ with $\mu_{0} < 1/2$ and let $k$, $t>0$ be such that
\begin{eqnarray}
\label{eq:AssumptionKT1}
k\mu(t) &<& 1/2\\
\frac{3t}{2-Q_{t}^{2}}  &<& 
\label{eq:AssumptionKT2}
\frac{4\loweralpha}{9\sigma_{\alpha}}
\end{eqnarray}
Then for small enough noise levels $\sigma$ one can find a regularization parameter $\lambda>0$ such that
\begin{equation}\label{eq:BoundsLambdaTh}
\frac{3}{2-Q_{t}^{2}}
\cdot \sqrt{t^{2} \sigma_{\alpha}^{2} + m\sigma^{2}}
\leq  \lambda \leq \frac 49 \loweralpha.
\end{equation}
Given $\sigma$ and $\lambda$ satisfying~(\ref{eq:BoundsLambdaTh}),  we define
\begin{equation}
\gamma \defin \frac{\lambda(2-Q_{t}^{2})}{\sqrt{5} \cdot \sqrt{t^{2} \sigma_{\alpha}^{2} + m\sigma^{2}}} \geq \sqrt{2\log2}.
\end{equation}
Let $\xb^{i} \in \Real^m$, $i \in \SET{n}$, where $n/\log n \geq mp$, be generated according to the signal model. 
Then, except with probability at most $\left(\frac{mpn}{9}\right)^{-mp/2} + \exp(-4n \cdot e^{-\gamma^{2}})$ we have
\begin{eqnarray}
\inf_{\Wb \in \Wcal_{\Dbo},\vb \in \Scal^{p}} \Delta F_{n}(\Wb,\vb,t)
&\geq &
(1 - \Kcal^2) \cdot \frac {\Exp[ \alpha_{0}^{2}]}{2} 
\cdot  
\frac{k}{p} \cdot t^{2}\notag\\
&&
-Q_t^2\left(\frac{16}{9} Q_{t}^2 + 3 \right)\cdot \Exp\{|\alpha_{0}|\} \cdot t \cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k\mu(t) \cdot \lambda \notag\\
&&
- A \cdot \gamma^{2} \cdot e^{-\gamma^{2}}\notag\\
&& -B \cdot \sqrt{mp \frac{\log n}{n}},
\end{eqnarray}
where
\begin{eqnarray}
\Kcal &\defin & C_{t} \cdot \big(\triple \Dbo \triple_2 \cdot \sqrt{k/p} + t\big)\\
A &\defin&
367 \cdot \left(t^{2}  \sigma_{\alpha}^{2} + 2m  \sigma^{2} + 2\lambda k\sigma_{\alpha}\right)\\
B &\defin &
3045 \left( k\sigma_{\alpha}^{2} \cdot t+2 m\sigma^{2} + 2\lambda k \sigma_{\alpha} \right).
\end{eqnarray}
\end{theorem}
Roughly speaking, the lower bound we obtain can be decomposed into three terms:
(1) the expected value of our surrogate function valid uniformly for all parameters $(\vb,\Wb)$,
(2) the contributions of the residual term (discussed in the next section) introducing the quantity $\gamma$,
and (3) the probabilisitc concentrations over the $n$ signals of the surrogate function and the residual term.

The proof of the theorem and its main building blocks are detailed in the next section.
%
%
\newpage
\section{Proof of Theorem~\ref{th:minimum_sparsecoding} and~\ref{th:minimum_sparsecoding_simple} }\label{app:minimum_sparsecoding}
We start with the more general theorem:
\subsection{Proof of Theorem~\ref{th:minimum_sparsecoding} }

We recall that we assume in Theorem~\ref{th:control_Fn} that
$
c_\lambda\cdot t  <
\frac{4\loweralpha}{9\sigma_{\alpha}}
$
and for small enough noise levels $\sigma$ one can find a regularization parameter $\lambda>0$ such that
\begin{equation*}
c_\lambda
\cdot \sqrt{t^{2} \sigma_{\alpha}^{2} + m\sigma^{2}}
\leq  \lambda \leq \frac 49 \loweralpha.
\end{equation*}
Given such $\sigma$ and $\lambda$, we define
$$
\gamma \defin  \frac{\lambda}{ c_\gamma  \sqrt{t^2 \sigma_\alpha^2 + m\sigma^2 } } \geq \sqrt{2\log(2)}.
$$
Here, $c_\lambda$ and $c_\gamma \defin \frac{\sqrt{5}}{3} c_\lambda$ stand for some universal constants which can be made explicit thanks to Theorem~\ref{th:control_Fn}.
\paragraph{Goal:} 
To determine when the lower bound proved in Theorem~\ref{th:control_Fn} is stricly positive, it is sufficient to consider when it holds that 
\begin{eqnarray*}
\Exp[\alpha^2]\cdot \frac{k}{p} \cdot t^2 &-& 
c_0 \lambda \cdot \Exp[|\alpha|]\cdot \frac{k}{p} \cdot t \cdot \triple \Dbo \triple_2 \cdot k \mu(t)\\
&-& c_1 (t^2\sigma_\alpha^2 + 2m\sigma^2 + 2 \lambda k \sigma_\alpha^2 )\cdot\gamma^2 e^{-\gamma^2}\\
%&-& c_2 (t k \sigma_\alpha^2 + 2m\sigma^2 + 2\lambda k \sigma_\alpha^2 ) \cdot \Lambda_n\quad\text{with}\quad
%\Lambda_n \defin \Big[ mp \frac{\log(n)}{n} \Big]^{\frac{1}{2}}\\
&\geq& t\cdot (-a_2 t^2 + a_1 t - a_0) > 0,
\end{eqnarray*}
for some universal constants $c_j$ which we can make explicit based on Theorem~\ref{th:control_Fn}, but which we keep hidden for clarity.


%\paragraph{Probability of success:} The probability of success of Theorem~\ref{th:control_Fn} is given by
%$$
%1 - \Big(\frac{mpn}{9}\Big)^{-mp/2} - \exp(-4ne^{-\gamma^2}).
%$$
%This induces a first condition over $\gamma$ (a upperbound), namely 
%\begin{equation*}
%ne^{-\gamma^2} \geq \epsilon_n\ \Rightarrow\ \gamma^2 \leq \log(n) - \log(\epsilon_n),\ \text{for some}\ 
%\epsilon_n \rightarrow \infty.
%\end{equation*}
%From now on, we make the choice 
%$\epsilon_n = \sqrt{n}$, so that $\exp(-4ne^{-\gamma^2}) \leq \exp(-4\sqrt{n})$, 
%along with the condition 
%\begin{equation}\label{eq:gamma_n}
% \gamma^2 \leq \frac{1}{2}\log(n).
%\end{equation}.

\paragraph{Noiseless/low-noise regime:}
Even though they are conceptually two different regimes, 
the treatment of the noisy and noiseless regimes follow the very same reasoning. From now on, we therefore assume that 
\begin{equation}\label{eq:noise}
m \sigma^2 \leq t^2 \sigma_\alpha^2,
\end{equation}
which determines the upper level of noise we will be able to handle. 

\paragraph{Second-order polynomial function in $t$:}
By simply using~(\ref{eq:noise}), $\lambda \leq \sqrt{2} c_\gamma \cdot \gamma \cdot \sigma_\alpha t$ and 
$3+2\sqrt{2} c_\gamma \leq 4\sqrt{2} c_\gamma$,
we now make explicit the $a_j$, $j \in \{0,1,2\}$, which define the second-order polynomial function in $t$:
\begin{eqnarray*}
a_2 & \defin & 3\sqrt{2} c_0 c_\gamma \cdot \sigma_\alpha\Exp[|\alpha|] \cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k \cdot \gamma\\
a_1 & \defin & \Exp[\alpha^2]\cdot \frac{k}{p} 
- \sqrt{2} c_0 c_\gamma \cdot \sigma_\alpha \Exp[|\alpha|]\cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k\mu_0 \cdot \gamma 
- 3c_1 \sigma_\alpha^2 \cdot \gamma^2 e^{-\gamma^2}\\
a_0 &\defin& 2\sqrt{2} c_\gamma \cdot k \sigma_\alpha^2\cdot[ c_1 \gamma^3 e^{-\gamma^2} + 2c_2\cdot \gamma\cdot \Lambda_n].
\end{eqnarray*}
We will make use of the following simple lemma to discuss the sign of this polynomial function:
\begin{lemma}\label{lem:poly}
Let $(a_0,a_1,a_2) \in \Real_+^3$.
If $4 a_0 a_2 < a_1^2$, and
$
t \in  \big[ \frac{2a_0}{a_1}, \frac{a_1}{2a_2} \big],
$
then 
$-a_2 t^2 + a_1 t - a_0 > 0$.
\end{lemma}
\paragraph{Some key definitions:}
Let $\theta$ be defined as 
$$
\theta \defin \min\bigg\{ \frac{\loweralpha}{\sigma_\alpha}, \frac{1}{3c_0} \cdot \frac{\Qcal_\alpha}{k \cdot \triple \Dbo \triple_2} \bigg\}.
$$
We also define $\gamma_{\min} > 1$ the unique number such that 
\begin{equation}\label{eq:gamma_min}
\gamma_{\min}^4 e^{-\gamma_{\min}^2} \defin \frac{q_\alpha}{69 c_1 c_\gamma^2} 
\cdot \frac{1}{p} \cdot \theta,  
\end{equation}
and
\begin{equation}\label{eq:gamma_max}
\gamma_{\max} \defin \frac{1}{2}
\min\bigg\{\sqrt{2\log(n)},
\frac{1}{2\sqrt{2} c_0 c_\gamma} \cdot
\frac{\Qcal_\alpha}{ k \mu_0\cdot \triple \Dbo \triple_2}\bigg\}.
\end{equation}
Moreover, we consider
\begin{equation}\label{eq:Lambda_max}
\Lambda_{n,\max} \defin \frac{q_\alpha}{138 c_2 c_\gamma^2} 
\cdot \frac{1}{p \cdot \gamma^2} \cdot \theta,  
\end{equation}

\paragraph{First step, non-emptiness of $[\gamma_{\min},\gamma_{\max}]$:}
We first check that the interval $[\gamma_{\min},\gamma_{\max}]$ is not empty.
On the one hand, if the value of $\gamma_{\max}$ is obtained by $\sqrt{1/2 \log(n)}$, 
we use the fact that $\gamma_{\min} < \gamma_{\max}$ is equivalent to $\gamma_{\min}^4 e^{-\gamma_{\min}^2} >  \gamma_{\max}^4 e^{-\gamma_{\max}^2}$.
In particular, we have
$$
 \gamma_{\max}^4 e^{-\gamma_{\max}^2} = \frac{\log^2(n)}{4\sqrt{n}} < \gamma_{\min}^4 e^{-\gamma_{\min}^2}, 
$$
a condition that will be implied by the more stringent condition $\Lambda_n \leq \Lambda_{n,\max}$.

On the other hand, and in the second scenario for $\gamma_{\max}$, we conclude based on the following lemma:
\begin{lemma}\label{lem:ineq_lambert}
Let $a>1$ and $b \in (0,1/5]$.
If 
$
a^4 e^{-a^2} = b 
$,
then 
$ 
\sqrt{\log(1/b)} \leq a \leq 2\sqrt{\log(1/b)}.
$
\end{lemma}
The sufficient condition which stems form this lemma reads
$$
k \mu_0\cdot \triple \Dbo \triple_2 \leq \frac{1}{4\sqrt{2} c_0 c_\gamma}\cdot \frac{\Qcal_\alpha}
{\sqrt{\log\big( 69 c_1 c_\gamma^2 \cdot \frac{1}{q_\alpha} 
\cdot \frac{p}{\theta}  \big)}}.
$$
\paragraph{Second step, lower bound on $a_1$:}
For any $\gamma \in [\gamma_{\min},\gamma_{\max}]$, it is first easy to check that 
$$
\sqrt{2} c_0 c_\gamma \cdot \sigma_\alpha \Exp[|\alpha|]\cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k\mu_0 \cdot \gamma 
\leq \frac{1}{4} \Exp[\alpha^2]\cdot \frac{k}{p}.
$$
Moreover, since $\gamma^2 e^{-\gamma^2} \leq \gamma^4 e^{-\gamma^2}$ and 
$
\frac{1}{12 c_1} q_\alpha \cdot \frac{k}{p} > \gamma_{\min}^4 e^{-\gamma_{\min}^2} , 
$
we therefore obtain that 
$$
a_1 \geq \Exp[\alpha^2]\cdot \frac{k}{p} - \frac{1}{4}\cdot \Exp[\alpha^2]\cdot \frac{k}{p} - \frac{1}{4}\cdot \Exp[\alpha^2]\cdot \frac{k}{p}
\geq \frac{1}{2} \cdot \Exp[\alpha^2]\cdot \frac{k}{p}.
$$
\paragraph{Third step, the condition $4a_0a_2 < a_1^2$:}
Since we have $a_1 > \frac{1}{2} \cdot \Exp[\alpha^2]\cdot \frac{k}{p}$, and 
$$
a_2 \leq 4\sqrt{2} c_\gamma \cdot k \sigma_\alpha^2\cdot \max\Big\{ c_1 \gamma^3 e^{-\gamma^2}, 2c_2\cdot \gamma\cdot \Lambda_n\Big\},
$$
simple computations show that 
$
\gamma \geq \gamma_{\min}
$
and 
$
\Lambda_n \leq \Lambda_{n, \max}
$, as defined in~(\ref{eq:gamma_min}) and (\ref{eq:Lambda_max}), lead to $4a_0a_2 < a_1^2$.
\paragraph{Conclusions:}
We have proved that for $\gamma \in [\gamma_{\min},\gamma_{\max}]$, 
$
\Lambda_n \leq \Lambda_{n, \max}
$,
and
$$
k \mu_0\cdot \triple \Dbo \triple_2 \leq \frac{1}{4\sqrt{2} c_0 c_\gamma}\cdot \frac{\Qcal_\alpha}
{\sqrt{\log\big( 69 c_1 c_\gamma^2 \cdot \frac{1}{q_\alpha} 
\cdot \frac{p}{\theta}  \big)}},
$$
the lower bound provided by Theorem~\ref{th:control_Fn} is stricly positive 
for a radius $t \in \big[ \frac{2a_0}{a_1}, \frac{a_1}{2a_2} \big]$ (see Lemma~\ref{lem:poly})
and a noise $\sigma \leq \sigma_\alpha \sqrt{m} t$.
Taking the smallest allowed radius (i.e., $t=\frac{2a_0}{a_1}$ with $\gamma = \gamma_{\max}$) leads to the displayed result.
%
%
\subsection{Proof of Theorem~\ref{th:minimum_sparsecoding_simple} }
We now discuss the version of Theorem~\ref{th:minimum_sparsecoding} in the simpler setting where there is no noise (i.e., $\sigma=0$)
and $\alphabo$ is almost surely bounded by $\upperalpha \geq \loweralpha > 0$.
The main consequence of these simplifying assumptions is that there is no residual term to consider anymore and our surrogate function 
coincide almost surely with the true sparse coding function, provided the radius $t$ is small enough,
as proved in Proposition~\ref{prop:simplified_exact_recovery}.
As a result, the terms depending on $\gamma$ in Theorem~\ref{th:control_Fn} disappear, and the probability of success simplifies to
$$
1 - \Big(\frac{mpn}{9}\Big)^{-mp/2}.
$$
Moreover, in light of Proposition~\ref{prop:simplified_exact_recovery}, we now ask for
\begin{equation*}
\frac{1}{3} c_\lambda \sqrt{k} \upperalpha t \leq \lambda \leq \frac 49 \loweralpha. 
\end{equation*}
The backbone of the proof remains identical, we
adapt the discussion about the polynomial function in $t$.
%
%
\paragraph{Goal:} 
To determine when the lower bound proved in Theorem~\ref{th:control_Fn} is stricly positive, it is sufficient to consider when it holds that 
\begin{eqnarray*}
\Exp[\alpha^2]\cdot \frac{k}{p} \cdot t^2 &-& 
c_0 \lambda \cdot \Exp[|\alpha|]\cdot \frac{k}{p} \cdot t \cdot \triple \Dbo \triple_2 \cdot k \mu(t)\\
&-& c_1 (t k \sigma_\alpha^2 + 2\lambda k \sigma_\alpha^2 ) \cdot \Lambda_n\quad\text{with}\quad
\Lambda_n \defin \Big[ mp \frac{\log(n)}{n} \Big]^{\frac{1}{2}}\\
&\geq& t\cdot (-a_2 t^2 + a_1 t - a_0) > 0,
\end{eqnarray*}
for some universal constants $c_j$ which we can make explicit based on Theorem~\ref{th:control_Fn}, but which we keep hidden for clarity.
\paragraph{Second-order polynomial function in $t$:}
By making the choice $\lambda \defin \frac{1}{2} c_\lambda \cdot \upperalpha \cdot \sqrt{k} \cdot t$,
we now make explicit the $a_j$, $j \in \{0,1,2\}$, which define the second-order polynomial function in $t$:
\begin{eqnarray*}
a_2 & \defin & \frac{3}{2} c_0 c_\lambda \cdot \upperalpha\cdot \Exp[|\alpha|] \cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k^{3/2} \\
a_1 & \defin & \Exp[\alpha^2]\cdot \frac{k}{p} 
- \frac{1}{2} c_0 c_\lambda \cdot \upperalpha\cdot \Exp[|\alpha|]\cdot \frac{k}{p} \cdot \triple \Dbo \triple_2 \cdot k^{3/2} \mu_0 \\
a_0 &\defin& 2 c_1 c_\lambda \cdot k^{3/2} \sigma_\alpha \upperalpha \cdot \Lambda_n.
\end{eqnarray*}
%
%
\paragraph{Conclusions:}
Consider the condition
$$
\triple \Dbo \triple_2\cdot k^{3/2}\mu_0 
\leq 
\frac{1}{c_0 c_\lambda} \frac{\Exp[\alpha^2]}{\upperalpha\cdot \sigma_\alpha},
$$
so that $a_1 \geq \frac{1}{2} \cdot \Exp[\alpha^2]\cdot \frac{k}{p}$.
By using again Lemma~\ref{lem:poly}, and by defining 
$$
\Lambda_{n,\max} \defin \frac{1}{9 c_1 c_\lambda^2} \cdot \frac{\Exp[\alpha^2]}{\upperalpha^2}
\cdot \frac{1}{k p} \cdot 
\min\bigg\{ \frac{\loweralpha}{\sigma_\alpha}, \frac{1}{5c_0} \cdot \frac{\Qcal_\alpha}{k \cdot \triple \Dbo \triple_2} \bigg\},
$$
it is easy to check that $\Lambda_n \leq \Lambda_{n,\max} $ implies that 
$4 a_0 a_2 < a_1^2$ along with 
$$
2 \frac{a_0}{a_1} < \frac{8}{9 c_\lambda} \frac{\loweralpha}{\upperalpha} \cdot \frac{1}{\sqrt{k}},
$$
as required by our choice of $\lambda$ and the fact that $\lambda \leq \frac{4}{9} \loweralpha$.
%
%

